Is the Observable Universe Consistent with the Cosmological Principle?

The Cosmological Principle (CP) -- the notion that the Universe is spatially isotropic and homogeneous on large scales -- underlies a century of progress in cosmology. It is conventionally formulated through the Friedmann-Lema\^itre-Robertson-Walker (FLRW) cosmologies as the spacetime metric, and culminates in the successful and highly predictive $\Lambda$-Cold-Dark-Matter ($\Lambda$CDM) model. Yet, tensions have emerged within the $\Lambda$CDM model, most notably a statistically significant discrepancy in the value of the Hubble constant, $H_0$. Since the notion of cosmic expansion determined by a single parameter is intimately tied to the CP, implications of the $H_0$ tension may extend beyond $\Lambda$CDM to the CP itself. This review surveys current observational hints for deviations from the expectations of the CP, highlighting synergies and disagreements that warrant further study. Setting aside the debate about individual large structures, potential deviations from the CP include variations of cosmological parameters on the sky, discrepancies in the cosmic dipoles, and mysterious alignments in quasar polarizations and galaxy spins. While it is possible that a host of observational systematics are impacting results, it is equally plausible that precision cosmology may have outgrown the FLRW paradigm, an extremely pragmatic but non-fundamental symmetry assumption.

==> Cosmological Principle Review/authors-observation.tex <==

\author{Pavan Kumar Aluri}
\affiliation{Department of Physics, Indian Institute of Technology (BHU), Varanasi - 221005, India }
% ORCID: 0000-0002-4333-9819

\author{Paolo Cea} 
\affiliation{INFN - Sezione di Bari, Via Amendola 173 - 70126 Bari, Italy} 
% ORCID: 0000-0001-5267-1461

\author{Pravabati Chingangbam}
\affiliation{Indian Institute of Astrophysics, Koramangala II Block, Bangalore 560 034, India}
\affiliation{School of Physics, Korea Institute for Advanced Study, 85 Hoegiro, Dongdaemun-gu, Seoul, 02455, Korea}
% ORCID: 

\author{Ming-Chung Chu}
\affiliation{Department of Physics and Institute of Theoretical Physics, The Chinese University of Hong Kong\\Shatin, Hong Kong}
% ORCID: 0000-0002-1971-0403

\author{Roger G. Clowes}
\affiliation{Jeremiah Horrocks Institute, University of Central Lancashire, Preston PR1 2HE, UK} 
% ORCID: 0000-0001-8370-465X

%\author{Carlos Frajuca}
%\affiliation{IMEF, FURG, Brazil}
% ORCID: 0000-0001-8463-3451

\author{Damien Hutsem{\'e}kers}
\affiliation{F.R.S.-FNRS, Institut d'Astrophysique et de G{\'e}ophysique (B5c), University of Li{\`ege}, 4000 Li{\`ege} Belgium}

\author{Joby P. Kochappan}
\affiliation{Asia Pacific Center for Theoretical Physics, Pohang, 37673, Korea}
% ORCID: 0000-0001-8849-3986

%\author{Andrzej Krasi\'nski}
%\affiliation{Nicolaus Copernicus Astronomical %Center, Polish Academy of Sciences, Bartycka 18, 00-%716 Warsaw, Poland}
% ORCID: 0000-0003-4947-3557

\author{Alexia M. Lopez} 
\affiliation{Jeremiah Horrocks Institute, University of Central Lancashire, Preston PR1 2HE, UK}
% ORCID: 0000-0003-4634-3124 (is this correct??)

\author{Lang Liu}
\affiliation{Department of Physics, Kunsan National University, Kunsan 54150, Korea}
% ORCID: 0000-0002-0297-9633

\author{Niels C. M. Martens}
\affiliation{Lichtenberg Group for History and Philosophy of Physics, University of Bonn, Germany}
\affiliation{Institute for Theoretical Particle Physics and Cosmology, RWTH Aachen University, Germany}
% ORCID: 0000-0002-2839-1387

\author{C.~J.~A.~P.~Martins}
\address{Centro de Astrof\'{\i}sica da Universidade do Porto, Rua das Estrelas, 4150-762 Porto, Portugal}
\address{Instituto de Astrof\'{\i}sica e Ci\^encias do Espa\c co, CAUP, Rua das Estrelas, 4150-762 Porto, Portugal}
% ORCID: 0000-0002-4886-9261

\author{Konstantinos Migkas}
\affiliation{Argelander-Institut f\"{u}r Astronomie, Universit\"{a}t Bonn, Auf dem H\"{u}gel 71, 53121 Bonn, Germany}
% ORCID: 0000-0003-0451-0449

\author{Eoin \'O Colg\'ain}
\affiliation{Atlantic Technological University, Ash Lane, Sligo, Ireland}
\affiliation{CQUeST \& Department of Physics, Sogang University, Seoul 121-742, Korea}
% ORCID: 0000-0003-0813-5156

\author{Pratyush Pranav}
\affiliation{Univ Lyon, ENS de Lyon, Univ Lyon1, CNRS, Centre de Recherche Astrophysique de Lyon UMR5574, F–69007, Lyon, France}
% ORCID: 0000-0003-0813-5156

\author{Lior Shamir}
\affiliation{Kansas State University, Manhattan, KS 66506, United States }
% ORCID: 0000-0002-6207-1491

\author{Ashok K. Singal}
\affiliation{Astronomy and Astrophysics Division, Physical Research Laboratory, Navrangpura, Ahmedabad - 380 009, India }
% ORCID: 0000-0002-8479-7656

\author{M. M. Sheikh-Jabbari}
\affiliation{School of Physics, Institute for Research in Fundamental Sciences (IPM),\\ P.O.Box 19395-5531, Tehran, Iran}
\affiliation{The Abdus Salam ICTP, Strada Costiera 11, I-34014, Trieste, Italy}
% ORCID: 0000-0002-3728-230X

%\author{Jiro Soda}
%\affiliation{Department of Physics, Kobe University,\\  Kobe 657-8501, Japan}
% ORCID: 0000-0003-1738-4605

%\author{Christos G. Tsagas}
%\affiliation{Section of Astrophysics, Astronomy and %Mechanics, Department of Physics Aristotle University of Thessaloniki, Thessaloniki 54124, Greece}
%\affiliation{Clare Hall, University of Cambridge, Herschel Road, Cambridge CB3 9AL, UK}
% ORCID: 0000-0002-8527-0418

\author{Jenny Wagner}
\affiliation{Bahamas Advanced Study Institute and Conferences, 4A Ocean Heights, Hill View Circle, Stella Maris, Long Island, The Bahamas}
% ORCID: 0000-0002-4999-3838

\author{Shao-Jiang Wang}
\affiliation{CAS Key Laboratory of Theoretical Physics, Institute of Theoretical Physics, Chinese Academy of Sciences, Beijing 100190, China}
% ORCID: 0000-0003-4378-870X

\author{David L. Wiltshire}
\affiliation{School of Physical \& Chemical Sciences, University of Canterbury, Private Bag 4800, Christchurch 8140, New Zealand}
% ORCID: 0000-0003-1992-6682

\author{Shek Yeung}
\affiliation{Department of Physics and Institute of Theoretical Physics, The Chinese University of Hong Kong\\Shatin, Hong Kong}

\author{Lu Yin}
\affiliation{CQUeST \& Department of Physics, Sogang University, Seoul 121-742, Korea}
% ORCID: 0000-0002-8289-0814

\author{Wen Zhao}
\affiliation{CAS Key Laboratory for Researches in Galaxies and Cosmology, Department of Astronomy, University of Science and Technology of China, Chinese Academy of Sciences, Hefei, Anhui 230026, China \\ School of Astronomy and Space Science, University of Science and Technology of China, Hefei, 230026, China}
% ORCID: 0000-0002-1330-2329
